Overcoming Failures of Imagination in AI Infused System Development and Deployment

NeurIPS 2020 requested that research paper submissions include impact statements on "potential nefarious uses and the consequences of failure." However, as researchers, practitioners and system designers, a key challenge to anticipating risks is overcoming what Clarke (1962) called 'failures of imagination.' The growing research on bias, fairness, and transparency in computational systems aims to illuminate and mitigate harms, and could thus help inform reflections on possible negative impacts of particular pieces of technical work. The prevalent notion of computational harms -- narrowly construed as either allocational or representational harms -- does not fully capture the open, context dependent, and unobservable nature of harms across the wide range of AI infused systems.The current literature focuses on a small range of examples of harms to motivate algorithmic fixes, overlooking the wider scope of probable harms and the way these harms might affect different stakeholders. The system affordances may also exacerbate harms in unpredictable ways, as they determine stakeholders' control(including of non-users) over how they use and interact with a system output. To effectively assist in anticipating harmful uses, we argue that frameworks of harms must be context-aware and consider a wider range of potential stakeholders, system affordances, as well as viable proxies for assessing harms in the widest sense.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> table-org.tex <==
\begin{table}[h!]
\scriptsize
    \centering
    \begin{tabular}{p{6.6cm}|p{7cm}}
         \hline\multicolumn{2}{c}{\small{\textbf{Concerning themes}}} \\\hline
         \small{\textbf{Theme}} &  \small{\textbf{Examples \&  references}} 
         \\\hline
         %
         \textbf{Research subject narrowly bounds the plane of inquiry}
         (e.g., fairness papers only describing positive contributions, theory papers suggesting they are exempt form reflections on impact, without offering a convincing argument). %Readers may wish to be convinced that a theoretical add-on does not itself create a possibility of, for example, a bias via disparate error rate leaking through. Just saying 'this work is theoretical' is not convincing enough.
         
         & ``At this point [this work] is theoretical and conceptual in nature and so is
its likely current broader impact.'' \cite{vialard2020shooting} ;\newline
``This study is crucial as it indicates the vulnerability of deep neural network (DNN) classifiers to adversarial attacks.'' \cite{dolatabadi2020advflow}
    \\\hline
         %
         \textbf{Emphasizing the \textit{net} impact of the paper} (i.e., righting the wrongs, attempting to defend, de-emphasize, or `balance' harms with unrelated benefits) 
         
         &
         ``However, we believe that the positive impact of foundational research on public datasets, such as is presented in this paper, far outweighs
these risks lying further downstream.'' \cite{asano2020labelling}
 \\\hline
         %
         \textbf{Outsourcing the ethical responsibility} 
	to previous or later stages in the algorithm development / use (e.g., references to `biased inputs', `mistakes of engineers', or `malicious intent of users' without further elaboration or discussion of created theoretical/technical affordances for misuse)
 
 &  
 ``[..] there exist risks that some engineers [..] can deliberately use the algorithm [..] which may actually harm the performance of the designed system.''\cite{hu2020one}
 \\\hline
         
        %
        
        \textbf{Neglect of some stakeholders} (typically those with least power). \\
	-- Assuming 'benefits' to mean benefits for the company / government / other 
agency that already has power.\\ 
	-- Assuming 'harms' to mean harms to the successful implementation / spread of the technology, or threats to the party that implements it. \newline
	-- Assuming `bad intentions' to be those of the users (and not agents with more power).
	-- Using terms like `reliable', `secure' without specifying: reliable \textit{for who}? Not addressing conflicts of interest.\linebreak
	-- Conceiving of `harm' solely in relation to war, government, or other `mass disaster' threats. Neglecting the severity and importance of individual harms.
	
	&
	 ``[..]there exist risks that some engineers [..] can deliberately use the algorithm [..] which may actually harm the performance of the designed system.'' %; ``[..] our work can bring both beneficial and harmful impacts and it really depends on the motivation of the users.'' 
	  \cite{hu2020one};
	 \newline
	 ``[..] this work remains largely academic in nature, and does not pose
foreseeable risks regarding defense, security, and other sensitive fields.'' \cite{aksan2020cose}; %they *did* mention more down-to-earth examples later
	\\\hline
	%
	\textbf{Assuming that the technical goals always have positive valence}
	(e.g., a gain in performance according to a particular metric is taken to be a good thing without further questioning)
	
	&
	
	\\\hline
	%
	\textbf{Using the Impact Statement as a sales pitch} or a recap of technical advances

	&
	\cite{ryu2020metaperturb, gan2020large, choromanski2020ode, dolatabadi2020advflow}
	
	\\\hline
	%
	\textbf{Assuming that wide adoption always has positive valence}

	&
	
	\\\hline
	%
	\textbf{Focusing on the ethics of \textit{research methods}} (and not the impact of findings, their use, and implications).

	&
	
	\\\hline
	%
	\textbf{ Overconfidence / not acknowledging epistemic uncertainty} (e.g. ascertaining no harm).
	&
	``If the method
fails in some extreme circumstances, it will confuse researchers or engineers [..]
but it will not bring about any negative ethical or societal consequences.''%; ``our method did not leverage biases in the data since we conduct experiments on datasets that are more about animals or pieces of equipment in the office.'' 
\cite{wang2020transferable}
	\\\hline
	%
	\multicolumn{2}{c}{\small{\textbf{Encouraging themes}}} \\\hline
	%
	\textbf{Admitting uncertainty} \newline
	-- Clearly stating epistemic limitations of envisioning positive and negative impacts\newline
	-- Promoting involvement of domain experts
	
	&
	``The present work is primarily theoretical, making its broader impact difficult to ascertain.‘’ \cite{pfau2020disentangling}; \newline
	``Performing meaningful probabilistic inferences requires some level of domain expertise regarding modeling priors and potential biases of sampling/variational approximations.'' \cite{pleiss2020fast}
	\\\hline
	%
	 \textbf{Considering various stakeholders}, situating the harms on micro and macro levels (environmental, economic, individual)
	
	&
	``Future work may [..] allow those without significant funding and computing power (e.g. researchers in non-R1 universities and small companies) to train neural networks of higher utility.'' \cite{dogra2020optimizing}\newline
	``We summarize the potential impact of our work in the following aspects.[..]To the research community [..] To the downstream engineers [..] To the society''\cite{hu2020one}
	\\\hline
	%
	 \textbf{Interrogating \textit{within} known benefits} \newline
	 -- Interrogating within a known fairness or accountability issue (e.g., examining whether better interpretability can lead to harm via advancing stereotypes)\newline
	 -- Examining weaknesses of technological improvements

	&
	``While we believe increasing the scalability and usability of these probabilistic techniques is a worthwhile goal, we note that they require additional care when using.[..] Calibration during model development must also be measured and iterated on. Failure to do this could lead to poor risk management in high risk applications.'', ``[..] some general risks associated with black-box optimization: a potential over-reliance on fully automated methods and computationally expensive searches for what might be marginal improvements.''
\cite{pleiss2020fast}
	\\\hline
	%
	\textbf{Naming particular examples} (application areas, tasks, failure scenarios, situations of harm)

	&
	``We should be cautious about the misuse
of the method proposed. [..] it might cause negative effect on democratic
privacy, e.g., Person ReID, Detection and etc.'' \cite{ren2020balanced};\newline
``Our method [..] can then be useful for [..] city planning, virtual tourism, and cultural heritage documentation [..]'', ``[..] might help identify and learn from rare organ disorders, when organs are represented as 3D point clouds.'', ``[..] potential to adversely impact people employed via crowd-sourcing sites [..] who manually review and annotate data.'' \cite{sharma2020self};\newline
``one mode of failure is when [quadrature approximations] fail to converge to a good estimate (for example, due to bad conditioning).''
\cite{pleiss2020fast}

	\\\hline
	%
    \end{tabular}
    \caption{Themes making frequent appearances in the 'Broader Impacts' statements from NeurIPS 2020 accepted papers.}
    \label{table:statement_themes_examples}
\end{table}
